TIGERScore: Towards Building Explainable Metric for All Text Generation Tasks

We present TIGERScore, a \textbf{T}rained metric that follows \textbf{I}nstruction \textbf{G}uidance to perform \textbf{E}xplainable, and \textbf{R}eference-free evaluation over a wide spectrum of text generation tasks. Different from other automatic evaluation methods that only provide arcane scores, TIGERScore is guided by natural language instruction to provide error analysis to pinpoint the mistakes in the generated text. Our metric is based on LLaMA-2, trained on our meticulously curated instruction-tuning dataset MetricInstruct which covers 6 text generation tasks and 23 text generation datasets. The dataset consists of 42K quadruple in the form of (instruction, input, system output $\rightarrow$ error analysis). We collected the `system outputs' through from a large variety of models to cover different types of errors. To quantitatively assess our metric, we evaluate its correlation with human ratings on 5 held-in datasets, 2 held-out datasets and show that TIGERScore can achieve the open-source SoTA correlation with human ratings across these datasets and almost approaches GPT-4 evaluator. As a reference-free metric, its correlation can even surpass the best existing reference-based metrics. To further qualitatively assess the rationale generated by our metric, we conduct human evaluation on the generated explanations and found that the explanations are 70.8\% accurate. Through these experimental results, we believe TIGERScore demonstrates the possibility of building universal explainable metrics to evaluate any text generation task. All the resourced are released in our project website: \url{https://tiger-ai-lab.github.io/TIGERScore/}.

==> figure/error_num_distribution.tex <==
\begin{figure}[h]
\centering
\resizebox{\linewidth}{!}{
\includesvg{figure/error_num_distribution.svg}
}
\caption{The distribution of the number of errors of the two channels.The horizontal axis shows the number of errors for an output.}
\label{fig:training_set_setting}
\end{figure}


==> figure/train_set_composition.tex <==
\begin{figure}[h]
\small
\resizebox{\linewidth/2}{!}{
\includesvg{figure/train_set_composition.svg}
}
\todo[inline]{TODO:other figure fill the line}
\caption{Composition of the training set, 31643 in total.}
\label{fig:training_set_setting}
\end{figure}


==> prompts/d2t.tex <==
\begin{verbatim}
Task instruction:${generation_instruction}
Source: ${input_context}
Reference 1: ${reference_output1}
...
Output: ${hypothesis_output}
\end{verbatim}
\begin{verbatim}
Based on the given Source and reference, identify the major and minor errors in this Output for the data to text task, which is to ${generation_instruction}. 
Note that Major errors refer to actual errors that affects the task severely, may change the meaning of the output, and Minor errors refer to smaller imperfections, and purely subjective opinions about the output. 
There may be multiple errors or no error in the output.
\end{verbatim}

==> prompts/ins.tex <==
\begin{verbatim}
Source: ${input_context or generation_instruction}
Reference: ${reference_output}
Output: ${hypothesis_output}
\end{verbatim}
\begin{verbatim}
Based on the given Source and reference, identify the major and minor errors in this Output for the ${task} task. Note that Major errors refer to actual errors that affects the task severely, may change the meaning of the output, and Minor errors refer to smaller imperfections, and purely subjective opinions about the output. You should check about ${aspects_list}.There may be multiple errors or no error in the output.
\end{verbatim}

==> prompts/json_2.tex <==
\begin{verbatim}
For each error identified above, please provide the following information in a specific JSON format:
- Error Location: The substring in the model-generated translation that contains the error.
- Error Aspect: Choose from ${aspect_descriptions}.
- Explanation: Describe why the identified issue is an error, and offer suggestions for correction. Explain as an expert in the task domain, without explicitly mentioning the reference output.
- Severity: Classify the error as "Major" or "Minor".
- Score Reduction: Assign a reduction score between 0.5 and 5, considering the severity of the error.

JSON Format for Output:
- If there are no errors:
```
{"errors": {}}
```
- If there are errors:
```
{"errors": {
"error_1": {
"error_location": "...",
"error_aspect": "...",
"explanation": "...",
"severity": "...",
"score_reduction": ...
},
...
}}
```
\end{verbatim}

==> prompts/lfqa.tex <==
\begin{verbatim}
Source: ${input_context}
Reference: ${reference_output}
Output: ${hypothesis_output}
\end{verbatim}
\begin{verbatim}
Based on the given Source and reference, identify the major and minor errors in this Output for the ${task} task, which is to ${generation_instruction}. Note that Major errors refer to actual errors that affects the task severely, may change the meaning of the output, and Minor errors refer to smaller imperfections, and purely subjective opinions about the output. You should check about ${aspects_lists}.There may be multiple errors or no error in the output.
\end{verbatim}

==> prompts/our_model_input_template.tex <==
\begin{verbatim}
You are evaluating errors in a model-generated output for a(an) ${task} task.
\end{verbatim}
\begin{verbatim}
Task instruction: ${generation_instruction}
Source: ${input_context}
Model-generated Output: ${hypothesis_output}

Based on the given task instruction and source, identify errors in this model-generated output.
For each error you give in the response, please also elaborate the following information:
- error location (the words that are wrong in the output)
- error aspect it belongs to.
- explanation why it's an error, and the correction suggestions.
- severity of the error ("Major" or "Minor"). 
- reduction of score (an interger between 1 and 5 given the severity of the error)

Your evaluation output:
\end{verbatim}

==> prompts/our_model_output.tex <==
\begin{verbatim}
The model-generated output contains ${total_penlty_numbers}$ errors, with a total score reduction of ${total_score_reduction}.
Error location 1: ${error_location}
Error aspect 1: ${error_aspect}
Explanation 1: ${explanation}
Severity 1: ${severity}
...
\end{verbatim}

==> prompts/summarization.tex <==
\begin{verbatim}
Source: ${input_context}
Reference: ${reference_output}
Output: ${hypothesis_output}
\end{verbatim}
\begin{verbatim}
Based on the given Source and Reference, please evaluate the quality of summary(Output) written for the input text. Please score the summarization with 0.5 to 5 for aspects below. Then, identify the major and minor errors in this output for the ${task} task. There may be multiple errors or no error in the output. Here are the aspects you need to focus on: 
${aspects_descriptions}
\end{verbatim}

==> prompts/translation.tex <==
\begin{verbatim}
Translation Instruction: ${generation_instruction}
Source Text: ${input_context}
${reference_output}
Model-generated Translation: ${hypothesis_output}

Please identify and categorize the errors in the model-generated translation as either Major or Minor. Major errors significantly impact the task, while Minor errors are subjective and represent minor imperfections.

When identifying errors, do not solely rely on the reference translation for comparison. Provide explanations as an expert in the task domain, without explicitly mentioning the reference output.
\end{verbatim}

==> tables/main_corr_results_3corrs_bak.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% \begin{table}
% \centering
% \vspace{-3em}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{@{}ccccccccc@{}}
% \toprule
% \multicolumn{1}{c|}{Tasks$\rightarrow$}                        & Summarization  & Translation    & Data2Text      & Long-form QA   & MathQA         & Inst-Fol       & \multicolumn{1}{c|}{Story-Gen}      & Average              \\
% \multicolumn{1}{c|}{Metrics$\downarrow$ Datasets$\rightarrow$} & SummaEval      & WMT22-zh-en    & WebNLG2020     & ASQA+          & gsm8k          & LIMA+          & \multicolumn{1}{c|}{ROC}            & \multicolumn{1}{l}{} \\ \midrule
% \multicolumn{9}{c}{Reference-based Metrics}                                                                                                                                                                                       \\ \midrule
% \multicolumn{1}{c|}{BLEU}                                      & 11.66          & 17.47          & 34.29          & 18.21          & 18.12          & 29.47          & \multicolumn{1}{c|}{-0.64}          & 18.37                \\
% \multicolumn{1}{c|}{ROUGE-2f}                                  & 16.03          & 16.26          & 35.85          & 19.66          & 20.69          & 33.49          & \multicolumn{1}{c|}{2.88}           & 20.69                \\
% \multicolumn{1}{c|}{InstructScore}                             & 27.40          & 51.55          & 47.28          & 20.59          & 0.36           & 20.98          & \multicolumn{1}{c|}{12.81}          & 25.85                \\
% \multicolumn{1}{c|}{GPTScore-ref}                              & 13.47          & 21.05          & 48.70          & 33.40          & 18.22          & 29.66          & \multicolumn{1}{c|}{18.94}          & 26.20                \\
% \multicolumn{1}{c|}{BARTScore-cnn (hypo-ref)}                   & 16.67          & 23.56          & 45.08 & 32.78          & 23.09          & 26.57          & \multicolumn{1}{c|}{27.61}          & 27.91                \\
% \multicolumn{1}{c|}{BARTScore-para (hypo-ref)}                 & 19.73          & 29.04          & 47.89          & 32.70          & 17.33          & 30.20          & \multicolumn{1}{c|}{17.76}          & 27.81                \\
% \multicolumn{1}{c|}{BERTScore}                                 & 26.26          & 37.65          & 48.22          & 26.39          & 11.19          & 45.58          & \multicolumn{1}{c|}{4.08}           & 28.48                \\
% \multicolumn{1}{c|}{BLEURT}                                    & 17.27          & 43.00          & \textbf{54.32} & 34.26          & 3.98           & 39.15          & \multicolumn{1}{c|}{27.89}          & 31.41                \\
% \multicolumn{1}{c|}{UniEval (summ)}                              & \textbf{53.22} & 23.11          & 51.14          & \textbf{36.95} & 17.69          & 30.87          & \multicolumn{1}{c|}{\textbf{44.88}} & 36.84                \\
% \multicolumn{1}{c|}{COMET-22}                                  & 35.32 & \textbf{58.46} & 43.82          & 36.79          & -5.58          & \textbf{49.68} & \multicolumn{1}{c|}{40.12}          & \textbf{36.94}       \\
% \multicolumn{1}{c|}{ChatGPT-prompting}                         & 45.53          & 43.77          & 47.76          & 29.84          & \textbf{61.26} & 15.36          & \multicolumn{1}{c|}{7.80}           & 35.90                \\ \midrule
% \multicolumn{9}{c}{Reference-free Metrics}                                                                                                                                                                                        \\ \midrule
% \multicolumn{1}{c|}{BARTScore-para (src-hypo)}                 & 43.11          & 6.96           & 37.82          & 29.86          & -0.41          & 19.37          & \multicolumn{1}{c|}{19.99}          & 22.38                \\
% \multicolumn{1}{c|}{BARTScore-cnn (src-hypo)}                  & 39.72          & 9.53           & 45.43          & 41.48          & 3.28           & 34.97          & \multicolumn{1}{c|}{\textbf{33.51}}          & 29.70                \\
% \multicolumn{1}{c|}{Llama-2-13b-chat-0-shot}                    & 29.59          & 9.09           & 41.32          & 21.67          & 2.80           & 22.71          & \multicolumn{1}{c|}{21.13}          & 21.19                \\
% \multicolumn{1}{c|}{COMETKiwi}                                 & 14.22          & \textbf{50.91} & 23.63          & 22.59          & -13.35         & 34.46          & \multicolumn{1}{c|}{19.12}          & 21.65                \\
% \multicolumn{1}{c|}{GPTScore-src}                              & 41.71 & 6.82           & 41.19 & 39.79          & 13.99          & 27.59          & \multicolumn{1}{c|}{23.22}          & 27.76                \\
% \midrule
% \multicolumn{1}{c|}{TigerScore-7B-V1.0}                        & \textbf{45.52}          & 34.52          & 50.35          & 42.45          & \textbf{33.44}          & 26.97          & \multicolumn{1}{c|}{29.97}          & 37.60                \\
% \multicolumn{1}{c|}{TigerScore-13B-V1.0}                       & 45.28          & \textbf{41.70}          & 49.02          & 45.91          & 30.68          & 36.92          & \multicolumn{1}{c|}{21.83}          & 38.76                \\
% \multicolumn{1}{c|}{TigerScore-7B-V1.2}                        & 43.95          & 37.70          & 49.13          & \textbf{46.10}          & 21.77          & 38.26          & \multicolumn{1}{c|}{39.90} & 39.54                \\
% \multicolumn{1}{c|}{TigerScore-13B-V1.2}                       & 44.21 & 41.54          & \textbf{52.87} & 44.76          & 24.41          & \textbf{47.52}          & \multicolumn{1}{c|}{\textbf{47.66}}          & \textbf{43.28}                \\ \midrule
% \multicolumn{1}{c|}{GPT4-0-shot}                                & 40.75          & 33.92          & 46.83          & 49.30 & 54.98 & 60.45 & \multicolumn{1}{c|}{37.74} & 46.28  \\
% \bottomrule

% \end{tabular}
% }
% \caption{The Pearson Correlation results of all the baseline metrics.}
% \label{tab:main_corr_results_3corrs_1}
% \vspace{1em}


% \resizebox{\linewidth}{!}{
% \begin{tabular}{@{}ccccccccc@{}}
% \toprule
% \multicolumn{1}{c|}{Tasks$\rightarrow$}                        & Summarization  & Translation    & Data2Text      & Long-form QA   & MathQA         & Inst-Fol       & \multicolumn{1}{c|}{Story-Gen}      & Average              \\
% \multicolumn{1}{c|}{Metrics$\downarrow$ Datasets$\rightarrow$} & SummaEval      & WMT22-zh-en    & WebNLG2020     & ASQA+          & gsm8k          & LIMA+          & \multicolumn{1}{c|}{ROC}            & \multicolumn{1}{l}{} \\ \midrule
% \multicolumn{9}{c}{Reference-based Metrics}                                                                                                                                                                                       \\ \midrule
% \multicolumn{1}{c|}{BLEU}                                      & 11.98          & 19.73          & 33.29          & 11.38          & 21.12          & \textbf{46.61} & \multicolumn{1}{c|}{-1.17}          & 20.42                \\
% \multicolumn{1}{c|}{ROUGE-2f}                                  & 14.53          & 17.83          & 35.49          & 16.83          & 22.12          & 44.56          & \multicolumn{1}{c|}{2.34}           & 21.96                \\
% \multicolumn{1}{c|}{InstructScore}                             & 26.33          & 50.43          & 38.54          & 21.62          & -4.15          & 16.19          & \multicolumn{1}{c|}{16.13}          & 23.58                \\
% \multicolumn{1}{c|}{GPTScore-ref}                              & 14.73          & 24.95          & 39.42          & 31.60          & 18.20          & 33.14          & \multicolumn{1}{c|}{18.24}          & 25.75                \\
% \multicolumn{1}{c|}{BARTScore-cnn (hypo-ref)}                   & 13.64          & 28.53          & 36.12 & 29.57          & 23.35          & 32.49          & \multicolumn{1}{c|}{26.64}          & 27.19                \\
% \multicolumn{1}{c|}{BARTScore-para (hypo-ref)}                 & 17.18          & 33.72          & 40.79          & 28.94          & 17.27          & 34.47          & \multicolumn{1}{c|}{17.43}          & 27.11                \\
% \multicolumn{1}{c|}{BERTScore}                                 & 23.67          & 42.41          & 43.75          & 25.60          & 11.53          & 45.77          & \multicolumn{1}{c|}{2.88}           & 27.95                \\
% \multicolumn{1}{c|}{BLEURT}                                    & 17.30          & 48.41          & \textbf{48.76} & 33.26          & 3.53           & 36.46          & \multicolumn{1}{c|}{27.52}          & 30.75                \\
% \multicolumn{1}{c|}{UniEval (summ)}                              & \textbf{47.52} & 21.90          & 38.38          & \textbf{41.83} & 19.78          & 16.02          & \multicolumn{1}{c|}{\textbf{44.46}} & 32.84                \\
% \multicolumn{1}{c|}{COMET-22}                                  & 33.75 & \textbf{56.35} & 33.92          & 35.28          & -5.53          & 46.13 & \multicolumn{1}{c|}{39.20}          & 34.16       \\
% \multicolumn{1}{c|}{ChatGPT-prompting}                         & 38.50          & 40.53          & 40.20          & 29.33          & \textbf{66.46} & 23.20          & \multicolumn{1}{c|}{4.77}           & \textbf{34.71}       \\ \midrule
% \multicolumn{9}{c}{Reference-free Metrics}                                                                                                                                                                                        \\ \midrule
% \multicolumn{1}{c|}{BARTScore-para (src-hypo)}                 & 38.68          & 9.60           & 32.26          & 26.86          & -2.70          & 5.92           & \multicolumn{1}{c|}{20.55}          & 18.74                \\
% \multicolumn{1}{c|}{BARTScore-cnn (src-hypo)}                  & 35.50          & 12.83          & 34.33          & 40.96          & 1.50           & 25.43          & \multicolumn{1}{c|}{33.48}          & 26.29                \\
% \multicolumn{1}{c|}{Llama-2-13b-chat-0-shot}                    & 28.53          & 14.38          & 29.24          & 19.91          & 1.08           & 21.37          & \multicolumn{1}{c|}{26.78}          & 20.18                \\
% \multicolumn{1}{c|}{COMETKiwi}                                 & 16.27          & \textbf{48.48} & 27.90          & 18.05          & -11.48         & 34.86          & \multicolumn{1}{c|}{18.47}          & 21.79                \\
% \multicolumn{1}{c|}{GPTScore-src}                              & 37.41 & 8.90           & 28.82 & 39.48          & 14.25          & 26.46          & \multicolumn{1}{c|}{24.35}          & 25.61                \\
% \midrule
% \multicolumn{1}{c|}{TigerScore-7B-V1.0}                        & 39.32          & 42.27          & 38.42          & 42.04          & \textbf{32.07}          & 25.53          & \multicolumn{1}{c|}{30.22}          & 35.69                \\
% \multicolumn{1}{c|}{TigerScore-13B-V1.0}                       & \textbf{41.98} & \textbf{45.20}          & 39.05          & 45.84          & 31.04          & 43.69          & \multicolumn{1}{c|}{17.40}          & 37.12                \\
% \multicolumn{1}{c|}{TigerScore-7B-V1.2}                        & 35.11          & 41.50          & 42.39          & \textbf{47.11 }         & 21.23          & 43.57          & \multicolumn{1}{c|}{39.26} & 38.60                \\
% \multicolumn{1}{c|}{TigerScore-13B-V1.2}                       & 36.81 & 44.99          & \textbf{45.88} & 46.22          & 23.32          & \textbf{47.03}          & \multicolumn{1}{c|}{\textbf{46.36}}          & \textbf{41.52}                \\ \midrule
% \multicolumn{1}{c|}{GPT4-0-shot}                                & 36.46          & 43.87          & 44.04          & 48.95 & 51.71 & 58.53 & \multicolumn{1}{c|}{32.48} & 45.15      \\
% \bottomrule
% \end{tabular}
% }
% \caption{The Spearman Correlation results of all the baseline metrics.}
% \label{tab:main_corr_results_3corrs_2}

% \vspace{1em}

% \resizebox{\linewidth}{!}{
% \begin{tabular}{@{}ccccccccc@{}}
% \toprule
% \multicolumn{1}{c|}{Tasks$\rightarrow$}                        & Summarization  & Translation    & Data2Text      & Long-form QA   & MathQA         & Inst-Fol       & \multicolumn{1}{c|}{Story-Gen}      & Average              \\
% \multicolumn{1}{c|}{Metrics$\downarrow$ Datasets$\rightarrow$} & SummaEval      & WMT22-zh-en    & WebNLG2020     & ASQA+          & gsm8k          & LIMA+          & \multicolumn{1}{c|}{ROC}            & \multicolumn{1}{l}{} \\ \midrule
% \multicolumn{9}{c}{Reference-based Metrics}                                                                                                                                                                                       \\ \midrule
% \multicolumn{1}{c|}{BLEU}                                      & 8.71           & 14.50          & 23.13          & 7.73           & 17.25          & 35.92 & \multicolumn{1}{c|}{-0.89}          & 15.19                \\
% \multicolumn{1}{c|}{ROUGE-2f}                                  & 10.67          & 13.19          & 24.74          & 11.73          & 18.07          & 34.59          & \multicolumn{1}{c|}{1.78}           & 16.40                \\
% \multicolumn{1}{c|}{InstructScore}                             & 20.86          & 40.44          & 30.21          & 15.64          & -3.87          & 13.87          & \multicolumn{1}{c|}{13.50}          & 18.66                \\
% \multicolumn{1}{c|}{GPTScore-ref}                              & 10.80          & 18.74          & 27.47          & 22.13          & 14.86          & 25.40          & \multicolumn{1}{c|}{12.78}          & 18.88                \\
% \multicolumn{1}{c|}{BARTScore-cnn (hypo-ref)}                   & 10.00          & 21.06          & 27.04 & 20.67          & 19.07          & 24.70          & \multicolumn{1}{c|}{18.58}          & 20.16                \\
% \multicolumn{1}{c|}{BARTScore-para (hypo-ref)}                 & 10.41          & 24.90          & 28.42          & 20.24          & 14.10          & 26.13          & \multicolumn{1}{c|}{12.11}          & 19.47                \\
% \multicolumn{1}{c|}{BERTScore}                                 & 17.39          & 31.57          & 30.74          & 17.70          & 9.41           & 35.61          & \multicolumn{1}{c|}{2.00}           & 20.63                \\
% \multicolumn{1}{c|}{BLEURT}                                    & 12.69          & 36.12          & \textbf{34.48} & 23.11          & 2.88           & 27.94          & \multicolumn{1}{c|}{19.18}          & 22.34                \\
% \multicolumn{1}{c|}{UniEval (summ)}                              & \textbf{35.89} & 16.08          & 28.56          & \textbf{29.32} & 16.15          & 11.93          & \multicolumn{1}{c|}{\textbf{31.22}} & 24.17                \\
% \multicolumn{1}{c|}{COMET-22}                                  & 25.01 & \textbf{42.79} & 23.43          & 24.66          & -4.52          & \textbf{36.17} & \multicolumn{1}{c|}{27.52}          & 25.01       \\
% \multicolumn{1}{c|}{ChatGPT-prompting}                         & 30.45          & 32.30          & 30.38          & 20.91          & \textbf{58.57} & 17.73          & \multicolumn{1}{c|}{3.26}           & \textbf{27.65}       \\ \midrule
% \multicolumn{9}{c}{Reference-free Metrics}                                                                                                                                                                                        \\ \midrule
% \multicolumn{1}{c|}{BARTScore-para (src-hypo)}                 & 29.12          & 7.01           & 22.32          & 18.80          & -2.21          & 4.26           & \multicolumn{1}{c|}{14.15}          & 13.35                \\
% \multicolumn{1}{c|}{BARTScore-cnn (src-hypo)}                  & 26.63          & 9.40           & 23.69          & 28.93          & 1.23           & 19.09          & \multicolumn{1}{c|}{23.29}          & 18.89                \\
% \multicolumn{1}{c|}{Llama-2-13b-chat-0-shot}                    & 25.22          & 11.79          & 23.45          & 15.96          & 1.08           & 19.50          & \multicolumn{1}{c|}{21.52}          & 16.93                \\
% \multicolumn{1}{c|}{COMETKiwi}                                 & 11.87          & 36.37 & 19.08          & 12.23          & -9.38          & 26.46          & \multicolumn{1}{c|}{12.78}          & 15.63                \\
% \multicolumn{1}{c|}{GPTScore-src}                              & 28.20 & 6.50           & 19.81 & 27.64          & 11.64          & 20.04          & \multicolumn{1}{c|}{16.36}          & 18.60                \\
% \midrule
% \multicolumn{1}{c|}{TigerScore-7B-V1.0}                        & 32.84          & 34.42          & 30.06          & 31.56          & \textbf{30.90}          & 23.24          & \multicolumn{1}{c|}{24.41}          & 29.63                \\
% \multicolumn{1}{c|}{TigerScore-13B-V1.0}                       & \textbf{36.09} & \textbf{37.13} & 31.34          & \textbf{34.18}          & 24.90          & 38.63          & \multicolumn{1}{c|}{13.15}          & 30.77                \\
% \multicolumn{1}{c|}{TigerScore-7B-V1.2}                        & 28.79          & 33.65          & 32.44          & 33.93          & 19.98          & 38.13          & \multicolumn{1}{c|}{29.72} & 30.95                \\
% \multicolumn{1}{c|}{TigerScore-13B-V1.2}                       & 31.29 & 36.50          & \textbf{36.43} & 33.17          & 21.58          & \textbf{41.84}          & \multicolumn{1}{c|}{\textbf{35.33}}          & \textbf{33.73 }               \\
% \midrule
% \multicolumn{1}{c|}{GPT4-0-shot}                                & 29.32          & 35.38          & 32.26          & 35.85 & 46.63 & 49.50 & \multicolumn{1}{c|}{25.69} & 36.38  \\
% \bottomrule
% \end{tabular}
% }
% \caption{The Kendall's tau Coefficient results of all the baseline metrics.}
% \label{tab:main_corr_results_3corrs_3}

% \end{table}

==> tables/overall_rating.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\begin{tabular}{@{}lccccc@{}}
\toprule
\multicolumn{1}{c}{Task$\downarrow$ Rate$\rightarrow$} & 1  & 2           & 3           & 4  & 5            \\ \midrule
Sum                                                    & 3  & 10          & \textbf{17} & 7  & 13           \\
Trans                                                  & 3  & 6           & 15          & 9  & \textbf{17}  \\
D2T                                                    & 11 & 10          & 4           & 7  & \textbf{18}  \\
LF-QA                                                  & 6  & 8           & 10          & 6  & \textbf{20}  \\
MathQA                                                 & 4  & 9           & 10          & 13 & \textbf{14}  \\
Instruct                                               & 9  & 4           & 3           & 7  & \textbf{27}  \\
StoryGen                                               & 7  & \textbf{12} & 11          & 9  & 11           \\ \midrule
Total                                                  & 43 & 59          & 70          & 58 & \textbf{120} \\ \bottomrule
\end{tabular}
\end{table}

==> tables/synthesis_data.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[]
\begin{tabular}{@{}lll@{}}
\toprule
Task                  & Aspects                                                                                                                               & Errors                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             \\ \midrule
Summarization         & \begin{tabular}[c]{@{}l@{}}Relevance,\\ Fact Consistency,\\ Coherence,\\ Fluency\end{tabular}                                         & \begin{tabular}[c]{p{9cm}@{}l@{}}This aspect refers to the degree to which the summarized output accurately reflects the key points of the input text. It assesses if the summary contains the necessary information from the original text. Example error types include: (1) Including irrelevant information, (2) Omitting important information, (3) Overemphasis on less important details, (4) Under-representation of key points, (5) Misrepresentation of main ideas, etc.,\\ This aspect evaluates if the facts in the summary are consistent with the facts in the original text. It checks the accuracy of information presented in the summary. Example error types include: (1) Factual inaccuracies, (2) Misinterpretation, (3) Addition of non-existent facts, (4) Omission of factual information, etc.,\\ This aspect pertains to the logical and meaningful arrangement of ideas in the summary. It checks if the summary makes sense as a standalone text. Example error types include: (1) Illogical sequence of ideas, (2) Lack of clear connections between ideas, (3) Poor paraphrasing, (4) Lack of thematic unity, etc.,\\ This aspect reviews the model-generated output's use of language, including grammar, punctuation, and vocabulary that affect the quality of the sentences. Example error types include: (1) Spelling mistakes, (2) Grammatical errors, (3) Vocabulary misuse, (4) Style and tone inconsistencies, (5) Garbled characters, etc.\end{tabular}                           \\ \midrule
Translation           & \begin{tabular}[c]{@{}l@{}}Accuracy,\\ Fluency,\\ Terminology,\\ Style Matching\end{tabular}                                          & \begin{tabular}[c]{@{}l@{}}This aspect refers to the degree to which the translated text adheres to the original text, maintaining the same meaning, context and cultural nuances. Example error types include: (1) Literal translation, (2) Omission, (3) Addition, (4) Mistranslation, (5) False friends , etc.,\\ This aspect refers to how naturally the translation reads in the target language. It should not sound like a translation but like a text originally written in the target language. Example error types include: (1) Grammar mistakes, (2) Syntax errors, (3) Inappropriate language registe, (4) Use of unnatural expressions, (5) Inconsistent tense usage, etc.,\\ This aspect refers to the appropriate use of specific terms and jargon related to a particular field or industry. Example error types include: (1) Incorrect use of proper nouns, (2) Incorrect use of technical terms, (3) Incorrect use of abbreviations, (4) Incorrect date, time, currency, and number formats, etc.,\\ This aspect refers to the translator's ability to maintain the same style, tone, and voice as the original text. Example error types include: (1) Inconsistent style, (2) Inconsistent tone, (3) Inconsistent voice, etc.\end{tabular}                                                                                                                                                                                                                                                      \\ \midrule
Data to Text          & \begin{tabular}[c]{@{}l@{}}Accuracy,\\ Logical Coherence,\\ Fluency\end{tabular}                                                      & \begin{tabular}[c]{@{}l@{}}This aspect deals with the correctness of the information presented by the output. It checks if the output is factually accurate and matches with the information provided in the input. Example error types include: (1) Factual inaccuracies, (2) Misinterpretation, (3) Inaccurate Data Conversion, (4) Contradictory information, (5) Incorrect reasoning, etc.,\\ This aspect evaluates how well the output transforms structured data into a comprehensible, logical, and engaging text. Example error types include: (1) Illogical sequence, (2) Inconsistent facts, (3) Poor paraphrasing, (4) Inadequate explanation, (5) Overcomplication, etc.,\\ This aspect reviews the model-generated output's use of language, including grammar, punctuation, and vocabulary that affect the quality of the sentences. Example error types include: (1) Spelling mistakes, (2) Grammatical errors, (3) Vocabulary misuse, (4) Style and tone inconsistencies, (5) Garbled characters, etc.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                \\ \midrule
Long-form QA          & \begin{tabular}[c]{@{}l@{}}Accuracy,\\ Completeness,\\ Informativeness,\\ Clarity\end{tabular}                                        & \begin{tabular}[c]{@{}l@{}}This aspect evaluates the factual correctness of the answer. It checks if the information provided in the response is true and matches with the facts available from reliable sources. Example error types include: (1) Factual inaccuracies, (2) Misinterpretation, (3) Outdated information, (4) Contradictory information, (5) Incorrect inference, etc.,\\ This aspect checks if the response provided answers all parts of the question comprehensively. It evaluates if the answer leaves out any critical parts or details that were asked in the question. Example error types include: (1) Partial answer, (2) Omission of key details, (3) Lack of context, (4) Lack of depth, (5) Ignoring multi-part questions, etc.,\\ This aspect assesses the quality of the response in terms of how helpful it is for the user to understand the answer. It checks if the response is clear, concise, and easy to understand. Example error types include: (1) Redundancy, (2) Irrelevance, (3) Overuse of jargon, (4) Lack of examples, (5) Lack of sources, etc.,\\ This aspect assesses the readability and understandability of the response. Errors in this stage could lead to answers that are difficult to understand, despite being factually correct and based on accurate information synthesis. Example error types include: (1) Unclear language, (2) Poor organization, (3) Lengthy responses, (4) Unexplained jargon, (5) Grammar or spelling errors, etc.\end{tabular} \\ \midrule
Instruction Following & \begin{tabular}[c]{@{}l@{}}Comprehension,\\ Accuracy,\\ Infromativeness\\ Coherence\end{tabular}                                      & \begin{tabular}[c]{@{}l@{}}This aspect evaluates how well the output understands the given instruction. Example error types include: (1) Misinterpretation, (2) Inability to grasp complex instructions, (3) Failure to understand context, etc.,\\ This aspect measures the correctness of the output in relation to the instruction and the paired input context. Example error types include: (1) Inconsistent content with instruction and input, (2) Factual errors, (3) Misapplication of instructions, (4) Incorrect reasoning, etc.,\\ This aspect assesses the relevancy and usefulness of the information provided by the output. Example error types include: (1) Irrelevant information, (2) Insufficient information, (3) Overload of information, (4) Outdated information, (5) Repetitive information, etc.,\\ This aspect evaluates how logically the output flows and connects. Errors in this stage could lead to answers that are difficult to understand, despite being factually correct and based on accurate information synthesis. Example error types include: (1) Grammar or spelling errors, (2) Poor organization, (3) Illogical sequence, (4) Inappropriate tone or style, (5) Non-sequiturs, etc.\end{tabular}                                                                                                                                                                                                                                                                       \\ \midrule
MathQA                & \begin{tabular}[c]{@{}l@{}}Problem Understanding,\\ Problem Formulation,\\ Computing Accuracy,\\ Solution Interpretation\end{tabular} & \begin{tabular}[c]{@{}l@{}}This aspect assesses how well the output accurately comprehend the text-based description of the math problem. Example error types include: (1) Problem misinterpretation, (2) Neglect of information, (3) Incorrect identification of variables, (4) Overinterpretation (5) Incorrect Assumptions, etc.,\\ This aspect involves translating the problem from a textual form into a mathematical equation or set of equations that can be solved. Example error types include: (1) Incorrect formula usage, (2) Incorrect variable usage, (3) Incorrect operator usage, (4) Missing steps, (5) Misalignment with problem, etc.,\\ This aspect assesses the output's ability to perform the mathematical operations accurately to arrive at the correct solution. Example error types include: (1) Arithmetic errors, (2) Incorrect variable assignment, (3) Incorrect operation order, (4) Misuse of operation rules, etc.,\\ This involves the how well the output correctly interpret the solution of the problem in the context of the original problem statement. Example error types include: (1) Incorrect contextual interpretation, (2) Ignoring units of measurement (3) Not addressing all parts of the problem, etc.\end{tabular}                                                                                                                                                                                                                                            \\ \bottomrule
\end{tabular}
\end{table}

==> tables/train_setting.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\small
\centering
\begin{tabular}{@{}c|ccc@{}}
\toprule
Task                  & Real World               & Synthesis               & Total \\ \midrule
Summarization         & 4867                     & 400                     & 5267  \\
Translation           & 5708                     & 400                     & 6108  \\
Data2Text             & 5614                     & 400                     & 6014  \\
Long-Form QA          & 3352                     & 1146                    & 4498  \\
MathQA                & 1146                     & 200                     & 1346  \\
Instruction-following & 2248                     & 3750                    & 5998  \\
Total                 & 22935                    & 6296                    & 29231 
\end{tabular}
\caption{Samples from two channels}
\label{tab:train_settings}
\end{table}

==> tables/train_test_table.tex <==
% \begin{table}[!tb]
% \small
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l|cc|c|cc}
% \toprule
% Task                      & \multicolumn{2}{c|}{Real-World}                                      & Synthesis     & \# Samples            & Mix Ratio             \\
% \midrule
% \multirow{4}{*}{Summ}      & SummEval                     & 24 Systems$\dagger$                  & CNN/DM        & \multirow{4}{*}{5267} & \multirow{4}{*}{12:1} \\
%                           & Xsum                         & BRIO                                 & Xsum          &                       &                       \\
%                           & Newsroom                     & Pegasus                              & Gigaword      &                       &                       \\
%                           & Samsum                       & FLAN-T5-Base                         & Samsum        &                       &                       \\
% \midrule
% Trans                     & WMT2022                          & 18 Systems$\dagger$                  & WMT2022           & 6108                  & 14:1                  \\
% \midrule
% \multirow{3}{*}{D2T}      & WebNLG-2020                  & 16 Systems$\dagger$                  & Dart          & \multirow{3}{*}{6014} & \multirow{3}{*}{14:1} \\
%                           & WikiTableText                & FLAN-T5-xxl                          & WikiTableText &                       &                       \\
%                           & ToTTo                        & FLAN-T5-xxl                          & ToTTo         &                       &                       \\
% \midrule
% \multirow{4}{*}{LF-QA}    & ASQA                         & Vicuna-13B                       & ASQA          & \multirow{4}{*}{4498} & \multirow{4}{*}{3:1}  \\
%                           & FeTaQA                       & Vicuna-13B                       & FeTaQA        &                       &                       \\
%                           & CosmosQA                     & Vicuna-13B                       & Cosmos QA     &                       &                       \\
%                           & ELI5                         & FLAN-T5-base                         & ELI5          &                       &                       \\
% \midrule
% MathQA                    & GSM8K       & WizardMath-13B      & GSM8K/MathQA       & 3758 &  18:1 \\
% \midrule
% \multirow{2}{*}{Instruct} & \multirow{2}{*}{MixInstruct} & \multirow{2}{*}{11 systems$\dagger$} & LIMA/AlpacaFarm    & \multirow{2}{*}{5998} & \multirow{2}{*}{3:5}  \\
%                           &                              &                                      & OASST1/Guanaco/Dolly       &                       &                       \\
% \bottomrule
% \end{tabular}
% }
% \caption{
% The composition of our two-channel data. For the Real World channel, the output source with $\dagger$ means `the outputs are taken from the original dataset' while the others were generated by us with the specified model. We employ diverse beam search with the number of beam groups set as 5 to generate five candidate outputs for each input, in addition to Math QA, where we adopt top-p sampling with temperature 0.8 and top-p 0.95.
% }
% \label{tab:two_channel_compostion}
% \end{table}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[!tb]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}c|ccc|ccc@{}}
\toprule
\multirow{2}{*}{Task}     & \multicolumn{3}{c|}{Real-World}                                            & \multicolumn{3}{c}{Synthesis}                                         \\ \cmidrule(l){2-7} 
                          & Dataset                      & Output Source   & \# Sample             & Dataset              & Output Source      & \# Sample             \\ \midrule
\multirow{2}{*}{Sum}      & SummEval, XSum,              & \multirow{2}{*}{27 Systems} & \multirow{2}{*}{4867} & CNN/DM,XSum,         & \multirow{2}{*}{GPT-4} & \multirow{2}{*}{400}  \\
                          & Newsroom,SAMSum              &                     &                       & Gigaword,SAMSum      &                        &                       \\ \midrule
Trans                     & WMT                          & 18 Systems                 & 5708                  & WMT                  & GPT-4                  & 400                   \\ \midrule
\multirow{2}{*}{D2T}      & WebNLG-2020                  & \multirow{2}{*}{17 Systems} & \multirow{2}{*}{5614} & WikiTableText        & \multirow{2}{*}{GPT-4} & \multirow{2}{*}{400}  \\
                          & WikiTableText,ToTTo          &                     &                       & Dart,ToTTo           &                        &                       \\ \midrule
\multirow{2}{*}{LF-QA}    & ASQA,FeTaQA                  & \multirow{2}{*}{5 Systems}  & \multirow{2}{*}{3352} & ASQA,FeTaQA          & \multirow{2}{*}{GPT-4} & \multirow{2}{*}{1146} \\
                          & CosmosQA,ELI5                &                     &                       & Cosmos QA,ELI5       &                        &                       \\ \midrule
MathQA                    & GSM8K                        & 5 Systems                 & 3558                  & GSM8K,MathQA         & GPT-4                  & 200                   \\ \midrule
\multirow{2}{*}{Instruct} & \multirow{2}{*}{MixInstruct} & \multirow{2}{*}{11 Systems} & \multirow{2}{*}{2248} & LIMA,AlpacaFarm      & \multirow{2}{*}{GPT-4} & \multirow{2}{*}{3750} \\
                          &                              &                     &                       & OASST1,Guanaco,Dolly &                        &                       \\ \bottomrule
\end{tabular}
}
\caption{
The composition of our two-channel data. For synthesis data, the output is generated by asking GPT-4 to synthesize incorrect outputs that contain a few specific types of errors. 
}
\label{tab:two_channel_compostion}
\end{table}
